One Simple Trick for Improving the Performance of Energy-Limited Local Inference and Training

Energy supply and heat dissipation are two of the main challenges with modern GPU deployments. While typically discussed in the context of new datacenter constructions, the same constraints also apply to small form-factor consumer devices, such as the DGX spark. In workloads characterized by alternating compute-intensive tasks such as matmuls with memory-bound operations such as norms or cross-entropy, the compute-intensive parts might hit power and/or thermal limits and start throttling. In this short paper, we show that chunking the workload into smaller parts that alternate compute and memory in higher frequencies, these power and temperature spikes can be smoothed out, preventing throttling and resulting in considerably faster wall-clock time and reduced total energy consumption. We present several scenarios in which this effect can be exploited on a DGX Spark with up to 2% performance and energy improvements, and demonstrate that the same phenomenon also happens on less constrained systems, such as a multi-GPU server, albeit at significantly reduced effect size of 1-2%.

==> full_code.tex <==
\appendix
\onecolumn

\section{Full Reproduction Code}

The full reproduction code, can be found in Listing \ref{lst:chunked-benchmark}. Hardware metrics were collected using the NVIDIA System Management Interface (NVIDIA-SMI) \newline

\lstset{
    language=Python,
    basicstyle=\ttfamily\scriptsize,
    columns=fullflexible,
    keepspaces=true,
    showstringspaces=false,
    breaklines=true,
    frame=single,
    xleftmargin=0pt,
    aboveskip=2pt,
    belowskip=2pt
}

\begin{lstlisting}[caption={PyTorch implementation of the chunked benchmark used in our evaluation.},label={lst:chunked-benchmark},captionpos=b]
import torch, sys, time

M = 1024 * 32
N = 131072
K = 2048
chunks = int(sys.argv[1])

a = torch.rand((M, K), device="cuda", dtype=torch.bfloat16)
b = torch.rand((N, K), device="cuda", dtype=torch.bfloat16)
c = torch.zeros((M, N), device="cuda", dtype=torch.bfloat16)
d = torch.zeros((N, K), device="cuda", dtype=torch.bfloat16)

@torch.compile
def memory_bound(c):
    c[...] = torch.softmax(c, dim=-1)

@torch.compile
def abs_max_error(a, b):
    return torch.max(torch.abs(a - b))

def workload_chunked(a, b, c, d, chunks: int):
    cs = M // chunks
    for m in range(0, M, cs):
        slice = torch.matmul(a[m:m+cs, :], b.T, out=c[m:m+cs, :])
        memory_bound(slice)
        d = torch.addmm(d, slice.T, a[m:m+cs, :], out=d)
    return c, d

start = time.time()

c_r, d_r = workload_chunked(a, b, c, torch.zeros((N, K), device="cuda", dtype=torch.bfloat16), 1)

c_t, d_t = workload_chunked(a, b, c, torch.zeros((N, K), device="cuda", dtype=torch.bfloat16), chunks)

for i in range(10):
    for _ in range(10):
        workload_chunked(a, b, c, d, chunks)
    torch.cuda.synchronize()

events = [torch.cuda.Event(enable_timing=True) for i in range(4)]
i, count, first = 0, 0, True

start_event = torch.cuda.Event(enable_timing=True)
intermediate_events = [torch.cuda.Event(enable_timing=True) for i in range(1000)]

start_event.record()

while True:
    events[i].record()

    for r in range(10):
        intermediate_events[count*10+r].record()
        workload_chunked(a, b, c, d, chunks)

    events[i+1].record()
    i = (i + 2) % 4

    if not first:
        events[i+1].synchronize()
        iter_time = events[i].elapsed_time(events[i+1]) / 10

        print(f"Time: {iter_time:.2f}")
        print(f"FLOP/s: {4*M*N*K/iter_time/1_000_000_000:.2f} GFLOP/s")
    else:
        first = False

    count += 1
    if count == 100:
        torch.cuda.synchronize()
        break

print(f"Total time: {time.time() - start:.2f} seconds")
\end{lstlisting}
